Catch You and I Can: Revealing Source Voiceprint Against Voice Conversion

Voice conversion (VC) techniques can be abused by malicious parties to transform their audios to sound like a target speaker, making it hard for a human being or a speaker verification/identification system to trace the source speaker. In this paper, we make the first attempt to restore the source voiceprint from audios synthesized by voice conversion methods with high credit. However, unveiling the features of the source speaker from a converted audio is challenging since the voice conversion operation intends to disentangle the original features and infuse the features of the target speaker. To fulfill our goal, we develop Revelio, a representation learning model, which learns to effectively extract the voiceprint of the source speaker from converted audio samples. We equip Revelio with a carefully-designed differential rectification algorithm to eliminate the influence of the target speaker by removing the representation component that is parallel to the voiceprint of the target speaker. We have conducted extensive experiments to evaluate the capability of Revelio in restoring voiceprint from audios converted by VQVC, VQVC+, AGAIN, and BNE. The experiments verify that Revelio is able to rebuild voiceprints that can be traced to the source speaker by speaker verification and identification systems. Revelio also exhibits robust performance under inter-gender conversion, unseen languages, and telephony networks.

==> sections/5.relatedwork.tex <==
\section{Related Work}
%In this section, we briefly review the most related works on voice conversion and voice conversion detection.

\subsection{Voice Conversion (VC)}
VC techniques can be categorized into parallel VC and non-parallel VC according to whether they require parallel corpus for training.

\textbf{Parallel VC}.  
Typical VC training using parallel corpus works as follows. First, speech segments (e.g., frames) of the raw audio and the parallel audio with the same content are aligned and associated with each other. Then, the mapping from the source speaker characteristics to the target speaker characteristics is trained on these aligned features. Abe et al.~\cite{abe1988voice} proposed to create code vectors based on hard clustering using vector quantization (VQ) on the original and the target speaker features separately. Several subsequent works~\cite{shikano1991speaker, arslan1997voice, turk2006robust} tried to reduce the quantization error of VQ by using a fuzzy VQ based on soft clustering and the output is weighed according to the source speaker features. Wu et al.~\cite{wu2013exemplar} utilized a similar conversion method, but the output is directly a linear combination of the exemplars instead of the code vectors in the codebook. Stylianou et al.~\cite{stylianou1998continuous} proposed a continuous probabilistic transformation method based on Gaussian mixture models (GMMs). Toda et al.~\cite{toda2007voice} proposed to alleviate the over-smoothing effect of the GMM-based method with global variance. Nakashika et al.~\cite{nakashika2013voice} used deep belief nets (DBNs) to model the original and the target speaker in a high-order space and convert the raw audio using a neural network (NN). Sun et al.~\cite{sun2015voice} proposed to use a bidirectional long short-term memory-based recurrent neural network (BiLSTM) for conversion. 


\textbf{Non-Parallel VC}. Early non-parallel VC methods are mainly based on direct transformation, which directly transforms original features into target features without explicitly disentangling the speaker-dependent features from all features. For example, several attempts~\cite{zhang2008text, erro2010inca, song2013nonparallel, benisty2014nonparallel} have been made to adapt parallel VC to use non-parallel training sets by applying an additional procedure for linguistic unit alignment or model adaptation. Kaneko et al.~\cite{kaneko2018cyclegan} and Fang et al.~\cite{fang2018high} proposed to use the cycle-consistent adversarial network (CycleGAN) to directly transform the original features into target features. Kameoka et al.~\cite{kameoka2018stargan} used StarGAN to enable many-to-many voice conversion with a generator conditioned on the target speaker label. However, direct transformation-based VC methods can only convert audios into target speakers that are seen in the training process. 

To overcome this shortcoming, disentanglement-based methods are developed. Hsu et al.~\cite{hsu2016voice} proposed to use a variational auto-encoder (VAE) consisting of an encoder that learns speaker-independent features and a decoder that converts towards a specific speaker. Nakashika et al.~\cite{nakashika2016nonparallel} decomposed speech contents and phonetic features with a restricted Boltzmann machine-based probabilistic model. Hsu et al.~\cite{hsu2017voice} proposed to use variational autoencoding Wasserstein generative adversarial network (VAW-GAN), with VAE as the encoder and WGAN as the decoder. Saito et al.~\cite{saito2018nonparallel} directly utilized pretrained ASR and ASV to extract phonetic posteriorgrams (linguistic features) and d-vectors (speaker features). Tobing et al.~\cite{tobing2019nonparallel} proposed to use CycleVAE to improve the disentangling capability. Wu et al.~\cite{wu2020one} proposed VQVC to utilize vector quantization and instance normalization (IN) techniques for disentanglement. Later, they proposed VQVC+ to combine vector quantization with U-Net to produce high-quality audios~\cite{wu2020vqvcp}. Chou et al.\cite{chou2019one} disentangled speaker and content features with average pooling layer and IN, and combine them with adaptive instance normalization technique (AdaIN). Chen et al.~\cite{chen2021again} developed AGAIN that uses activation as an information bottleneck to further separate speaker features from content features. Liu et al.\cite{liu2021any} proposed BNE-Seq2seqMoL to extract content features with an encoder-decoder-based hybrid connectionist-temporal-classification-attention (CTC-attention) phoneme recognizer, of which the encoder has a bottleneck layer that outputs the content representations. Disentanglement-based methods have become a trend of real-time VC because non-parallel and one-shot conversion can be achieved. However, there is no way to obtain a model that can perfectly separate content and speaker features, thus leaving room to restore the voiceprint of the source speaker.

\subsection{Voice Conversion Detection}

Speech deepfake detection is one of the aims of the ASVspoof 2021 Challenge~\cite{yamagishi2021asvspoof} and is the main topic of the 2022 Audio Deep Synthesis Detection (ADD) Challenge~\cite{yi2022add}. Increasing efforts have been made to detect deepfake audios, of which VC-processed audios are a large part.

Tak et al.~\cite{tak2021end} proposed a spectro-temporal graph attention network (GAT) as the detection model that can learn cues across sub-bands and temporal intervals. Ge et al.~\cite{ge2021raw} proposed a differentiable architecture search method to automatically optimize the network architecture of the detection model. Chen et al.~\cite{chen2021pindrop} used a cascade of an embedding extractor and a backend classifier to improve the generalization of the detection model. Yi et al.~\cite{yi2021half} developed a training dataset for half-truth audio detection. Das et al.~\cite{das2021know} and Chen et al.~\cite{chen2021ur} augmented the audio data with MPEG-2, MPEG-3, MPEG-4, Ogg, True Audio (TTA), Windows Media Audio (WMA), Advanced Audio Coding (AAC) and Real Audio (RA) compression methods for the detection model. Tomilov et al.~\cite{tomilov2021stc} proposed to emulate the magnitude responses of codecs with randomly selected FIR filters. Leon et al.~\cite{leon2012evaluation} proposed to detect synthetic speech based on the relative phase shift (RPS) feature. Wang et al.~\cite{wang2020deepsonar} proposed to detect synthesized fake voices by monitoring neuron behaviors of the speaker recognition  system. Chen et al.~\cite{chen2020generalization} proposed to improve the generalization ability of the detection model with large margin cosine loss function (LMCL) and online frequency masking augmentation. Ma et al.~\cite{ma2021continual} proposed the method of detecting fake without forgetting (DFWF) to learn new spoofing attacks incrementally based on continual learning. Zhang et al.~\cite{zhang2021multi} used multi-task learning with SELCNN model to handle both segment-level and utterance-level features.

Nonetheless, existing works only aim at detecting whether the audio is genuine or fake, while we take a step further to restoring the voiceprint of the source speaker of a VC audio. 



==> tables/4VC-NT.tex <==
\begin{table}[tt]\centering
\begin{threeparttable}
% \renewcommand{\TPTminimum}{\linewidth}
\setlength{\abovecaptionskip}{5pt}% 
\setlength{\belowcaptionskip}{0pt}%

\caption{Performance of M1 against four VCs.}

\small
\setlength{\tabcolsep}{1.5mm}{
\begin{tabular}{@{}lrrrrr@{}}
\toprule
\multicolumn{2}{r}{\textbf{Training set}}                               & {VQ-Train}      & {V+-Train}          & {AG-Train}                     & {BN-Train}                 \\ \midrule
\multicolumn{2}{r}{\textbf{Test Set}}                                   & {VQ-Test}       & {V+-Test}           & {AG-Test}                      & {BN-Test}                  \\ \midrule
\multirow{2}{*}{\textbf{SV}}                & {Seen EER $\downarrow$\tnote{\textdaggerdbl}}     & 6.49\%          & 5.38\%              & 3.79\%                         & ?\%                                       \\
                                            & {Unseen EER $\downarrow$}              & 5.57\%          & 3.95\%              & 2.57\%                         & ?\%                                      \\ \midrule
\multirow{3}{*}{\textbf{SI}\tnote{\textdagger}}      & {Top-1~~ACC $\uparrow$}              & 91.35\%         & 95.03\%             & 97.66\%                        & ?\%                                      \\
                                            & {Top-5~~ACC $\uparrow$}              & 97.95\%         & 99.23\%             & 99.74\%                        & ?\%                                      \\
                                            & {Top-10~ACC $\uparrow$}              & 99.07\%         & 99.65\%             & 99.97\%                        & ?\%                                      \\ \bottomrule
\end{tabular}}              


\begin{tablenotes}[flushleft]
\footnotesize
\item[] \vspace{-1pt}\hspace{-2pt} \textdaggerdbl: Four training sets are partitioned into 9 to 1 (validation set). Seen EER is test on the validation set. 
\textdagger: Identification from 40 unseen speakers.

\end{tablenotes}

\label{tab:4vc-NT}
\end{threeparttable}
\end{table}

==> tables/4VC-T.tex <==
\begin{table}[tt]\centering
\begin{threeparttable}
% \renewcommand{\TPTminimum}{\linewidth}
\setlength{\abovecaptionskip}{5pt}% 
\setlength{\belowcaptionskip}{0pt}%

\caption{Performance of M3 against four VCs.}

\small
\setlength{\tabcolsep}{1.5mm}{
\begin{tabular}{@{}lrrrrr@{}}
\toprule
\multicolumn{2}{r}{\textbf{Training set}}                               & {VQ-Train}      & {V+-Train}          & {AG-Train}                     & {BN-Train}                 \\ \midrule
\multicolumn{2}{r}{\textbf{Test Set}}                                   & {VQ-Test}       & {V+-Test}           & {AG-Test}                      & {BN-Test}                  \\ \midrule
\multirow{2}{*}{\textbf{SV}}                & {Seen EER $\downarrow$\tnote{\textdaggerdbl}}     & 6.84\%          & 5.85\%              & 2.63\%                         & ?\%                                       \\
                                            & {Unseen EER $\downarrow$}                         & 4.08\%          & 3.35\%              & 1.87\%                         & 3.78\%                                      \\ \midrule
\multirow{3}{*}{\textbf{SI}\tnote{\textdagger}}      & {Top-1~~ACC $\uparrow$}                  & 93.21\%         & 95.93\%             & 99.07\%                        & 96.12\%                                      \\
                                            & {Top-5~~ACC $\uparrow$}                           & 98.62\%         & 99.36\%             & 99.94\%                        & 99.97\%                                      \\
                                            & {Top-10~ACC $\uparrow$}                           & 99.55\%         & 99.68\%             & 100.0\%                        & 100.0\%                                      \\ \bottomrule
\end{tabular}}              


\begin{tablenotes}[flushleft]
\footnotesize
\item[] \vspace{-1pt}\hspace{-2pt} \textdaggerdbl: Four training sets are partitioned into 9 to 1 (validation set). Seen EER is test on the validation set. 
\textdagger: Identification from 40 unseen speakers.

\end{tablenotes}

\label{tab:3vc-NT}
\end{threeparttable}
\end{table}

==> tables/4VC-T0.tex <==
\begin{table}[tt]\centering
\begin{threeparttable}
% \renewcommand{\TPTminimum}{\linewidth}
\setlength{\abovecaptionskip}{5pt}% 
\setlength{\belowcaptionskip}{0pt}%

\caption{Performance of M2 against four VCs.}

\small
\setlength{\tabcolsep}{1.5mm}{
\begin{tabular}{@{}lrrrrr@{}}
\toprule
\multicolumn{2}{r}{\textbf{Training set}}                               & {VQ-Train}      & {V+-Train}          & {AG-Train}                     & {BN-Train}                 \\ \midrule
\multicolumn{2}{r}{\textbf{Test Set}}                                   & {VQ-Test}       & {V+-Test}           & {AG-Test}                      & {BN-Test}                  \\ \midrule
\multirow{2}{*}{\textbf{SV}}                & {Seen EER $\downarrow$\tnote{\textdaggerdbl}}     & 6.96\%          & 6.18\%              & 2.78\%                         & ?\%                                       \\
                                            & {Unseen EER $\downarrow$}                         & 4.40\%          & 3.66\%              & 1.94\%                         & ?\%                                      \\ \midrule
\multirow{3}{*}{\textbf{SI}\tnote{\textdagger}}      & {Top-1~~ACC $\uparrow$}                  & 93.11\%         & 94.65\%             & 98.59\%                        & ?\%                                      \\
                                            & {Top-5~~ACC $\uparrow$}                           & 98.81\%         & 98.88\%             & 99.90\%                        & ?\%                                      \\
                                            & {Top-10~ACC $\uparrow$}                           & 99.87\%         & 99.55\%             & 99.97\%                        & ?\%                                      \\ \bottomrule
\end{tabular}}              


\begin{tablenotes}[flushleft]
\footnotesize
\item[] \vspace{-1pt}\hspace{-2pt} \textdaggerdbl: Four training sets are partitioned into 9 to 1 (validation set). Seen EER is test on the validation set. 
\textdagger: Identification from 40 unseen speakers.

\end{tablenotes}

\label{tab:4vc-T0}
\end{threeparttable}
\end{table}

==> tables/jiangbo.tex <==



\begin{table*}[tb]
	\renewcommand\arraystretch{1}
	\centering
	\small
	\caption{Feasibility of \sys attack on 8 camera systems.}
	\label{table:cameras}
	%	\setlength{\tabcolsep}{0.3mm}{	
		\begin{threeparttable}
			\resizebox{\linewidth}{!}{
				\begin{tabular}{|c|c|c|p{1.5cm}<{\centering}|p{1cm}<{\centering}|c|cc|ccc|c|c|}
					\hline
					\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Camera \\ Sytems\end{tabular}}} & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Manuf. \&\\ Model\end{tabular}}} & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Sensor  \\ (Type)\end{tabular}}} & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Max\\ Res.\end{tabular}}} & \multirow{2}{*}{\textbf{FPS}} & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Physically\\ Sealed\end{tabular}}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Attack\\ Parameters\tnote{\textdagger}\end{tabular}}}                                                                   & \multicolumn{3}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Manipulation of \\ Intra-frame Ribboning\end{tabular}}} & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Inter-frame\\ Stitching\tnote{\textdaggerdbl}\end{tabular}}} & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Attack\\ Scenarios \end{tabular}}} \\ \cline{7-11}
					&                                                                                     &                                                                                  &                                                                              &                               &                                                                                       & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Eff. Freq.\\ (MHz)\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}Max Dist.\\ (mm)\end{tabular}} & \multicolumn{1}{c|}{\textbf{Pos.}}         & \multicolumn{1}{c|}{\textbf{Wid.}}        & \textbf{Num.}        &                                                                                           &                                                                                      \\ \hline
					\multirow{7}{*}{IoT Kit}                                                          & \begin{tabular}[c]{@{}c@{}}Raspberry Pi\\ 3B+\end{tabular}                          & \begin{tabular}[c]{@{}c@{}}CMOS \\ (OmniVision OV5647)\end{tabular}                           & 2592*1944                                                                    & 30 fps                        & \XSolidBrush                                                                                   & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}20$-$110\\330$-$500\\ 740$-$1000\end{tabular}}                  & 82                                                                  & \multicolumn{1}{c|}{ \Checkmark}                   & \multicolumn{1}{c|}{ \Checkmark}                  &  \Checkmark                 &  \Checkmark                                                                                       & \begin{tabular}[c]{@{}c@{}}Object\\ Detection\end{tabular}                           \\ \cline{2-13} 
					& \begin{tabular}[c]{@{}c@{}}Arduino MKR \\ Vidor 4000\end{tabular}                   & \begin{tabular}[c]{@{}c@{}}CMOS \\ (Sony IMX219 NoIR)\end{tabular}                           & 3280*2464                                                                    & 30 fps                           & \XSolidBrush                                                                                   & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}30$-$100\\310$-$480\\ 740$-$1000\end{tabular}}                                                                   &80                                                                   & \multicolumn{1}{c|}{ \Checkmark}                   & \multicolumn{1}{c|}{ \Checkmark}                  &  \Checkmark                  &  \Checkmark                                                                                       & \begin{tabular}[c]{@{}c@{}}Object\\ Detection\end{tabular}                           \\ \cline{2-13} 
					& \begin{tabular}[c]{@{}c@{}}ASUS\\ Tinker Board 2\end{tabular}                        & \begin{tabular}[c]{@{}c@{}}CMOS \\ (Sony IMX219)\end{tabular}                           & 3280*2464                                                                    & 20 fps                        & \XSolidBrush                                                                                   & \multicolumn{1}{c|}{{\begin{tabular}[c]{@{}c@{}}30$-$90\\310$-$480\\ 720$-$1000\end{tabular}}}                                                                   &78                                                                   & \multicolumn{1}{c|}{ \Checkmark}                   & \multicolumn{1}{c|}{ \Checkmark}                  &  \Checkmark                  &  \Checkmark                                                                                       & \begin{tabular}[c]{@{}c@{}}Face\\ Detection\end{tabular}                             \\ \hline
					\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Dashboard\\ Camera\end{tabular}}                                                           & \begin{tabular}[c]{@{}c@{}}360 M320 \\ Dashcam\end{tabular}                         & CMOS (N/A)                                                                            & 2560*1440                                                                    & 25 fps                        &  \Checkmark                                                                                   & \multicolumn{1}{c|}{{\begin{tabular}[c]{@{}c@{}}520$-$630\\ 900$-$ 1000\end{tabular}}}                                                                   &40                                                                   & \multicolumn{1}{c|}{ \Checkmark}                   & \multicolumn{1}{c|}{ \Checkmark}                  &  \Checkmark                  &  \Checkmark                                                                                       & \begin{tabular}[c]{@{}c@{}}Object\\ Detection \end{tabular}                           \\ \cline{2-13} 
					& \begin{tabular}[c]{@{}c@{}}Blackview \\ Dashcam\end{tabular}                         & CMOS  (N/A)                                                                           & 2340*1296                                                                    & 30 fps                        &  \Checkmark                                                                                   & \multicolumn{1}{c|}{{\begin{tabular}[c]{@{}c@{}}520$-$620\\ 710$-$1000\end{tabular}}}                                                                   &75                                                                   & \multicolumn{1}{c|}{ \Checkmark}                   & \multicolumn{1}{c|}{ \Checkmark}                  &  \Checkmark                  &  \Checkmark                                                                                       & \begin{tabular}[c]{@{}c@{}}Object\\ Detection\end{tabular}                           \\ \hline
					IP Camera                                                                          & \begin{tabular}[c]{@{}c@{}}Xiaomi Dafang\\ IP Camera\end{tabular}                & \begin{tabular}[c]{@{}c@{}}1/2.7 Inch \\ CMOS (N/A)\end{tabular}                       & 1920*1080                                                                    & 15 fps                        &  \Checkmark                                                                                   & \multicolumn{1}{c|}{{\begin{tabular}[c]{@{}c@{}}100$-$500\\ 740$-$ 1000\end{tabular}}}                                                                   &32                                                                   & \multicolumn{1}{c|}{ \Checkmark}                   & \multicolumn{1}{c|}{ \Checkmark}                  &  \Checkmark                  &  \Checkmark                                                                                       & \begin{tabular}[c]{@{}c@{}}Face\\ Detection\end{tabular}                             \\ \hline
					\begin{tabular}[c]{@{}c@{}}Intelligent Access \\ Control System\end{tabular}              & \begin{tabular}[c]{@{}c@{}}Baidu Dumu\\ CM-mini\end{tabular}                        & \begin{tabular}[c]{@{}c@{}}1/2.7 Inch\\ Starlight CMOS (N/A) \end{tabular}              & 1920*1080                                                                    & 25 fps                           &  \Checkmark                                                                                   & \multicolumn{1}{c|}{{\begin{tabular}[c]{@{}c@{}}630$-$1000\end{tabular}}}                                                                   &15                                                                   & \multicolumn{1}{c|}{ \Checkmark}                   & \multicolumn{1}{c|}{ \Checkmark}                  &  \Checkmark                  &  \Checkmark                                                                                       & \begin{tabular}[c]{@{}c@{}}Face\\ Detection \end{tabular}                             \\ \hline
					Smart Phone                                                                        & \begin{tabular}[c]{@{}c@{}}Google Pixel\\ One\end{tabular}                          & \begin{tabular}[c]{@{}c@{}}CMOS (Sony \\ IMX1378 Exmor RS)\end{tabular}                  & 3840*2160                                                                    & 30 fps                        &  \Checkmark                                                                                   & \multicolumn{1}{c|}{{\begin{tabular}[c]{@{}c@{}}30$-$100\\ 740$-$1000\end{tabular}}}                                                                   & 18                                                                   & \multicolumn{1}{c|}{ \Checkmark}                   & \multicolumn{1}{c|}{ \Checkmark}                  &  \Checkmark                  &  \Checkmark                                                                                       & \begin{tabular}[c]{@{}c@{}}Face\\ Detection\end{tabular}                             \\ \hline
			\end{tabular}}
			\begin{tablenotes} 
				\footnotesize
				\item[\textdagger] The efficient frequency and the max attack distance are measured in our laboratory environment.
				\item[\textdaggerdbl] These camera systems are evaluated in two case studies: object detection and face detection.
			\end{tablenotes}
		\end{threeparttable}
		\vspace{-20pt}
\end{table*}

==> tables/threeVCs.tex <==
\begin{table}[tt]\centering
\begin{threeparttable}
% \renewcommand{\TPTminimum}{\linewidth}
\setlength{\abovecaptionskip}{5pt}% 
\setlength{\belowcaptionskip}{0pt}%

\caption{Voiceprint restoration performance against three VCs.}

\small
\setlength{\tabcolsep}{1.5mm}{
\begin{tabular}{@{}lrrrrr@{}}
\toprule
\multicolumn{2}{r}{\textbf{Training set}}                               & {VQ-Train}      & {V+-Train}          & {AG-Train}                     & {BN-Train}                 \\ \midrule
\multicolumn{2}{r}{\textbf{Test Set}}                                   & {VQ-test}       & {V+-test}           & {AG-test}                      & {BN-test}                  \\ \midrule
\multirow{2}{*}{\textbf{SV}}                & {Seen EER$^\ddagger$}     & 1.14\%          & 1.14\%              & 1.86\%                         & 3.90\%                                       \\
                                            & {Unseen EER}              & 10.24\%         & 10.24\%             & 4.22\%                         & 13.96\%                                      \\ \midrule
\multirow{3}{*}{\textbf{SI}$^\dagger$}      & {Top-1~~ACC}              & 89.62\%         & 89.62\%             & 98.53\%                        & 72.40\%                                      \\
                                            & {Top-5~~ACC}              & 96.54\%         & 96.54\%             & 99.87\%                        & 93.40\%                                      \\
                                            & {Top-10~ACC}              & 98.11\%         & 98.11\%             & 99.87\%                        & 97.47\%                                      \\ \bottomrule
\end{tabular}}              


\begin{tablenotes}[flushleft]
\item[] \vspace{-1pt}\hspace{-2pt}\footnotesize (i)$^\dagger$: Speakers in the SI task are all unseen. (ii)$^\ddagger$: Three training sets are partitioned into 9 to 1 (validation set). Seen EER is test on the validation set.
\end{tablenotes}

\label{tab:3vc}
\end{threeparttable}
\end{table}

==> tables/trans.tex <==
\begin{table*}\centering
\begin{threeparttable}[tt]
% \renewcommand{\TPTminimum}{\linewidth}
\setlength{\abovecaptionskip}{5pt}% 
\setlength{\belowcaptionskip}{0pt}%

\caption{Model transferability and capacity.}

\normalsize
\setlength{\tabcolsep}{2mm}{
\begin{tabular}{@{}lrrr|rr|rr|rrr@{}}
\toprule
\multicolumn{2}{r}{\textbf{Training set}}                    & \multicolumn{2}{c|}{VQ-Train} & \multicolumn{2}{c|}{AG-Train} & \multicolumn{2}{c|}{BN-Train} & \multicolumn{3}{c}{VAP-Train$^\dagger$} \\ \midrule
\multicolumn{2}{r}{\textbf{Test set}}                        & AG-Test       & BN-Test       & VQ-Test       & BN-Test       & VQ-Test       & AG-Test       & VQ-Test  & AG-Test  & BN-Test \\ \midrule
\textbf{SV}                  & {Unseen EER}           & 16.04\%       & 42.07\%       & 23.62\%       & 41.95\%       & 36.75\%       & 27.42\%       & 8.52\%   & 4.82\%   & 17.67\% \\ \midrule
\multirow{3}{*}{\textbf{SI}} & {Top-1~~ACC} & 67.08\%       & 1.44\%        & 45.19\%       & 1.67\%        & 8.17\%        & 31.60\%       & 89.07\%  & 98.43\%  & 62.05\% \\
                             & {Top-5~~ACC} & 90.96\%       & 19.17\%       & 75.71\%       & 21.03\%       & 30.93\%       & 64.30\%       & 97.50\%  & 99.78\%  & 88.08\% \\
                             & {Top-10~ACC}      & 95.83\%       & 35.90\%       & 87.24\%       & 39.78\%       & 49.55\%       & 78.75\%       & 99.07\%  & 99.97\%  & 94.23\% \\ \bottomrule
\end{tabular}}              


\begin{tablenotes}[flushleft]
\item[] \vspace{-1pt}\hspace{-2pt}\footnotesize (i)$^\dagger$: \textit{VAP-Train} consists of one-third of each of \textit{VQ-Train}, \textit{AG-Train} and \textit{BN-Train}. 
\end{tablenotes}

\label{tab:trans}
\end{threeparttable}
\end{table*}
